MINDFul.jl: A Framework for Intent-driven Multi-Domain Network coordination

Network coordination across multiple domains is a complex task that requires seamless communication among network entities. Network operators aim to minimize costs while ensuring the requirements of user requests are met. Such efforts are highly challenging in decentralized environments with diverse network operators, where only partial knowledge of the complete network is available. Intent-driven multi-domain coordination offers various benefits, some inherent to IBN and others stemming from the standardization of the NBI. As standardization is still missing, there has not been a substantial initiative to develop tools that leverage this paradigm. MINDFul.jl is a Julia library that provides a means to accelerate research in this area, at both the architectural and algorithmic levels. It provides a stateful, modular representation of common metro/core IP-optical network equipment as well as the common intent operations. Finally, it introduces a novel modular IBN-over-SDN architecture and is part of a library ecosystem that facilitates event-based simulations with a hackable interface and offers visualization support.

==> journal_dat.tex <==
% **************GENERATED FILE, DO NOT EDIT**************

\def\@journalName{}
\def\@volume{1}
\def\@issue{1}
\def\@year{2023}

